A Data Science Approach for Honeypot Detection in Ethereum

Ethereum smart contracts have recently drawn a considerable amount of attention from the media, the financial industry and academia. With the increase in popularity, malicious users found new opportunities to profit by deceiving newcomers. Consequently, attackers started luring other attackers into contracts that seem to have exploitable flaws, but that actually contain a complex hidden trap that in the end benefits the contract creator. In the blockchain community, these contracts are known as honeypots. A recent study presented a tool called HONEYBADGER that uses symbolic execution to detect honeypots by analyzing contract bytecode. In this paper, we present a data science detection approach based foremost on the contract transaction behavior. We create a partition of all the possible cases of fund movements between the contract creator, the contract, the transaction sender and other participants. To this end, we add transaction aggregated features, such as the number of transactions and the corresponding mean value and other contract features, for example compilation information and source code length. We find that all aforementioned categories of features contain useful information for the detection of honeypots. Moreover, our approach allows us to detect new, previously undetected honeypots of already known techniques. We furthermore employ our method to test the detection of unknown honeypot techniques by sequentially removing one technique from the training set. We show that our method is capable of discovering the removed honeypot techniques. Finally, we discovered two new techniques that were previously not known.

==> tables/numeric_distributions.tex <==
\begin{table*}[ht]
\centering
\caption{Distribution description for the most relevant numerical features. The normal transaction value mean is shown in ether.}
\label{table:numerical-distributions}
\begin{tabular}{|r|r|r|r|r|r|r|}
\hline
Feature & \multicolumn{2}{|c}{\textit{numSourceCodeLines}} &
\multicolumn{2}{|c}{\textit{normalTransactionCount}} &
\multicolumn{2}{|c|}{\textit{normalTransactionValueMean}} \\
\hline
Honeypot & Yes & No & Yes & No & Yes & No \\
\hline
%count &                         295.00 &  158568.00 &                   295.00 &    158568.00 &                        295.00 &  158568.00 \\
mean  &                          57.00 &     279.70 &                     5.13 &       680.61 &                          0.27 &       5.46 \\
std   &                          22.80 &     278.42 &                     4.26 &     33198.52 &                          0.22 &     570.30 \\
min   &                          19.00 &       1.00 &                     1.00 &         1.00 &                          0.00 &       0.00 \\
25\%   &                          41.00 &     109.00 &                     3.00 &         1.00 &                          0.10 &       0.00 \\
50\%   &                          54.00 &     177.00 &                     4.00 &         2.00 &                          0.25 &       0.00 \\
75\%   &                          67.00 &     386.00 &                     6.00 &         4.00 &                          0.38 &       0.00 \\
max   &                         185.00 &   11409.00 &                    32.00 &  10412943.00 &                          1.67 &  204365.82 \\
\hline
\end{tabular}
\end{table*}
